A Methodology to Determine Tooling Interface Temperature and Traction Conditions from Measured Force and Torque in Materials Processing Simulations Based on Multimesh Error Estimation

A methodology is presented for estimating average values for the temperature and the frictional traction over a tool-workpiece interface using measured values of force and torque applied to the tool. The approach was developed specifically for friction stir welding and friction stir processing applications, but is sufficiently general to be of use in a variety of other processes that involve sliding contact and heating at a tool-workpiece interface. The methodology works with a finite element framework that is intended to predict the evolution of the microstructural state of the workpiece material as it undergoes a complex thermomechanical history imposed by the process tooling. We employ a three-dimensional, Eulerian, finite element formulation; it includes coupling among the solutions for velocity, temperature and material state evolution. A critical element of the methodology is a procedure to estimate the tool interface traction and temperature from typical, measured values of force and torque. The procedure leads naturally to an intuitive basis for estimating error that is used in conjunction with multiple meshes to assure convergence. The methodology is demonstrate for a suite of three experiments that had been previously published as part of a study on the effect of weld speed on friction stir welding. The probe interface temperatures and torques are estimated for all three weld speeds and the multi-mesh error estimation methodology is employed to quantify the rate of convergence. Finally, comparison of computed and measured power usage is used as a further validation. Using the converged results, trends in the material flow, temperature, stress, deformation rate and material state with changing weld conditions are examined.

==> kocks-mecking.tex <==
%
%  Table:  Material Parameters
%
\begin{table}
    %
    \caption{Material parameters for constitutive model.{\bf  Correct the values for G }}
    \label{tab:MaterialParameters}
    \centering
    %
    \begin{tabular}{||c|c|c|c||} \hline
	\textbf{parameter}& \textbf{unit} & 
        \textbf{phase 1}  & \textbf{phase 2}  \\ \hline
                $G_0$     &  \GPa    &   43.4   & 43.4    \\ \hline
                $G_t$     &  \GPaPerK&   -0.021 & -0.021    \\ \hline
                $m_0$     & - &  0.05    & -0.685   \\ \hline
                $m_t$     & \perK &  0.0     & 7.0e-4   \\ \hline
                $Q/R$     & \degK  &  100.0   & 1.0e3    \\ \hline
                $\theta_0$  & \degK &   462.0  & 900.0    \\ \hline
                $D_0$  & \perSec &   1.0    & 1.0    \\ \hline
    \end{tabular}
    %
\end{table}
        


==> pStudy.tex <==
%
%  Table:  pStudy
%
\begin{table}
    %
    \caption{Parameter Study Results}
    \label{tab:pStudy}
    \centering
    %
    \begin{tabular}{||c|c||} \hline
	item1 & item2  \\ \hline
            1 &  2     \\ \hline
            1 &  2     \\ \hline
    \end{tabular}
    %
\end{table}


==> state-evolution.tex <==
%
%  Table:  State Variable Evolution
%
\begin{table}
    %
    \caption{Material parameters for state variable evolution.}
    \label{tab:StateEvolution}
    \centering
    %
    \begin{tabular}{||c|c|c|c||} \hline
	\textbf{parameter}   & \textbf{unit}  & \textbf{phase 1}  & \textbf{phase 2}  \\ \hline
                $a_s$      &  - &  0.17  & 0.304  \\ \hline
                $b_s$      &  - &  -0.02   & -0.185     \\ \hline
                $h_s$      &  \GPa  &  50.0   & 20.0 \\ \hline
                $n_s$      &  - &  1.0   &  1.0 \\ \hline
                $D_s$      & \perSec   &  $1.0\times 10^{7}$   & $1.0\times 10^{7}$ \\ \hline
                $\theta_r$  & \degK      &   1150   & 1150   \\ \hline
                $D_r$       & \perSec    &   1.0    & 1.0  \\ \hline
    \end{tabular}
    %
\end{table}
        


==> thermal-bcs.tex <==
%
%  Table:  thermal-bcs
%
\begin{table}
    %
    \caption{Boundary conditions for equations governing the  temperature field.}
    \label{tab:thermal-bcs}
    \centering
    %
    \begin{tabular}{||p{2.5in}|p{2.5in}||} \hline
	\textbf{surface}       &  \textbf{description} \\ \hline
            probe     &  fixed temperature; varies with parameter study\\ \hline
            inlet     &  temperature specified (\valUnit{300}{K}) \\ \hline
            outlet,  lateral A,   lateral R  &  zero heat flux \\ \hline
            top inside, top outside &  radiation to ambient temperature of \valUnit{300}{K}
                          with emissivity of 0.5 \\ \hline
            bottom inside, bottom outside  & convective heat transfer to ambient temperature of 300K
                             with coefficient of \valUnit{50}{W/(K ${\rm m}^2$)}\\ \hline
    \end{tabular}
    %
\end{table}


==> thermal-parameters.tex <==
%
%  Table:  Thermal Parameters
%
\begin{table}
    %
    \caption{Material constants for thermal problem.}
    \label{tab:thermal-parameters}
    \centering
    %
    \begin{tabular}{||c|c|c||} \hline
	\textbf{parameter} &\textbf{unit} & \textbf{value}  \\ \hline
            $\rho$       &kg/$\mbox{\textrm{m}}^3$  & 4430    \\ \hline
            $c_p$ &J/kg K &  533  \\ \hline
            $\kappa$    &W/mK     &    7.5    \\ \hline
    \end{tabular}
    %
\end{table}


==> velocity-bcs.tex <==
%
%  Table:  Velocity BCs
%
\begin{table}
    %
    \caption{Boundary conditions for equations governing the velocity field.
Degrees of freedom not explicitly mentioned are considered
as zero-valued traction components.}
    \label{tab:velocity-bcs}
    \centering
    %
    \begin{tabular}{||p{2.5in}|p{2.5in}||} \hline
	\textbf{surface}       &  \textbf{description} \\ \hline
            inlet     &  velocity specified in weld direction\\ \hline
            outlet     & zero traction\\ \hline
            probe     &  zero normal velocity; 
                         constant traction in direction of rotation
                         with magnitude derived to produce a given torque\\ \hline
            lateral surfaces, top and bottom & zero normal velocity \\ \hline
%            lateral A,
%            lateral R,
%            top inside,
%            top outside,
%            bottom inside,
%            bottom outside & zero normal velocity \\ \hline
    \end{tabular}
    %
\end{table}

